PointNeXt: Revisiting PointNet++ with Improved Training and Scaling Strategies

PointNet++ is one of the most influential neural architectures for point cloud understanding. Although the accuracy of PointNet++ has been largely surpassed by recent networks such as PointMLP and Point Transformer, we find that a large portion of the performance gain is due to improved training strategies, i.e. data augmentation and optimization techniques, and increased model sizes rather than architectural innovations. Thus, the full potential of PointNet++ has yet to be explored. In this work, we revisit the classical PointNet++ through a systematic study of model training and scaling strategies, and offer two major contributions. First, we propose a set of improved training strategies that significantly improve PointNet++ performance. For example, we show that, without any change in architecture, the overall accuracy (OA) of PointNet++ on ScanObjectNN object classification can be raised from 77.9% to 86.1%, even outperforming state-of-the-art PointMLP. Second, we introduce an inverted residual bottleneck design and separable MLPs into PointNet++ to enable efficient and effective model scaling and propose PointNeXt, the next version of PointNets. PointNeXt can be flexibly scaled up and outperforms state-of-the-art methods on both 3D classification and segmentation tasks. For classification, PointNeXt reaches an overall accuracy of 87.7 on ScanObjectNN, surpassing PointMLP by 2.3%, while being 10x faster in inference. For semantic segmentation, PointNeXt establishes a new state-of-the-art performance with 74.9% mean IoU on S3DIS (6-fold cross-validation), being superior to the recent Point Transformer. The code and models are available at https://github.com/guochengqian/pointnext.

==> figures/acc_flops.tex <==
% \begin{figure}[t] 
\begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-0.5em}
\centering
\includegraphics[width=0.5\textwidth]{static/teaser_acc_flops.png}
% \vspace{-.5em}
\caption{\textbf{Tradeoffs between Overall Accuracy on ScanObjectNN \cite{uy-scanobjectnn-iccv19} and GFLOPs}. The proposed PointNext outperforms the state-of-the-art with better accuracy, smaller model size, and less computation. Refer to \seclabel~\ref{sec:exp} for details. \protect\tikz[baseline]{\protect\draw[red, line width=0.5mm, dashed ] (0,.5ex)--++(0.45,0);} denotes the Accuracy-FLOPs curve of previous methods. The radius of each circle is portion to the number of parameters.
\GQ{add more models}
}
\label{fig:acc_flops}
\end{wrapfigure}
% \end{figure}



==> figures/resblock.tex <==
 \begin{wrapfigure}{r}{7cm}
%  \begin{figure}[t] 
\centering
\begin{subfigure}{0.24\textwidth}
\includegraphics[page=2, trim=0 3.6inch 8.3inch 0, clip,  height=35mm]{static/PointNextfig.pdf}
\caption{SA w/o subsampling}
\label{fig:resblock0}
\end{subfigure}
% \hfill
% \begin{subfigure}{0.24\textwidth}
% \includegraphics[page=3, trim=0 3.60inch 8.3inch 0, clip,  height=35mm]{static/PointNextfig.pdf}
% \caption{Separable SA}
% \label{fig:resblock2}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.24\textwidth}
% \includegraphics[page=4, trim=0 3.6inch 8.3inch 0, clip, height=35mm]{static/PointNextfig.pdf}
% \caption{Move up Separable SA}
% \label{fig:resblock3}
% \end{subfigure}
\hfill
\begin{subfigure}{0.24\textwidth}
\includegraphics[page=5, trim=0 3.6inch 8.3inch 0, clip, height=35mm]{static/PointNextfig.pdf}
\caption{InvResMLP}
\label{fig:resinvblock}
\end{subfigure}
\hfill
\caption{The step-by-step birth process of the proposed Inverted Residual MLPs (InvResMLP). InvResMLP stems from (a) the set abstraction module of PointNet++~\cite{qi2017pointnet2} while removing the subsampling layer. The MLPs are further separated into three parts as shown in (b) to make the computation efficient and to reinforce pointwise feature extraction. (c) The Move up Separable SA moves up the local aggregation part and achieves the same performance and speed as Seprable SA. (d) The InvResMLP is proposed by introducing the inverted bottleneck in the last two MLPs of (c). Note the (number) besides MLP in the figure denotes the channel size of output features. 
}
\label{fig:block}
% \end{figure}
\end{wrapfigure}
 
 


%%%% a birth progress of InvResMLP
 
%  \begin{figure}[t] 
% % \vspace{-0.5em}
% \centering
% \begin{subfigure}{0.24\textwidth}
% \includegraphics[page=2, trim=0 3.6inch 8.3inch 0, clip,  height=35mm]{static/PointNextfig.pdf}
% \caption{SA w/o subsampling}
% \label{fig:resblock0}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.24\textwidth}
% \includegraphics[page=3, trim=0 3.60inch 8.3inch 0, clip,  height=35mm]{static/PointNextfig.pdf}
% \caption{Separable SA}
% \label{fig:resblock2}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.24\textwidth}
% \includegraphics[page=4, trim=0 3.6inch 8.3inch 0, clip, height=35mm]{static/PointNextfig.pdf}
% \caption{Move up Separable SA}
% \label{fig:resblock3}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.24\textwidth}
% \includegraphics[page=5, trim=0 3.6inch 8.3inch 0, clip, height=35mm]{static/PointNextfig.pdf}
% \caption{InvResMLP}
% \label{fig:resinvblock}
% \end{subfigure}
% \hfill
% \caption{The step-by-step birth process of the proposed Inverted Residual MLPs (InvResMLP). InvResMLP stems from (a) the set abstraction module of PointNet++~\cite{qi2017pointnet2} while removing the subsampling layer. The MLPs are further separated into three parts as shown in (b) to make the computation efficient and to reinforce pointwise feature extraction. (c) The Move up Separable SA moves up the local aggregation part and achieves the same performance and speed as Seprable SA. (d) The InvResMLP is proposed by introducing the inverted bottleneck in the last two MLPs of (c). Note the (number) besides MLP in the figure denotes the channel size of output features. 
% }
% \label{fig:block}
% \end{figure}
 

==> sections/checklist.tex <==

\newpage

\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{All claims all accurately reflect the paper's contributions, and were validated in the \seclabel~\ref{sec:ablation}. }
  \item Did you describe the limitations of your work?
    \answerYes{The limitation was discussed at \seclabel~\ref{sec:limit}.} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Available in the \supp.} 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Our paper conforms to the ethics review guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Available in the \supp.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \seclabel~\ref{sec:exp} Experimental setups for optimization techniques and \seclabel~\ref{sec:ablation_train_strategies} for data augmentations used in training.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We reported all results with average and standard deviation in three random runs except the S3DIS 6-fold. We trained on all areas for three times, and picked the best on validation for each area, then performed the 6-fold cross-validation. Note that the averaged results with error bars on S3DIS area 5 are available in \tablabel~\ref{tab:ablate_s3dis} and \supp.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See \seclabel~\ref{sec:exp} Experimental setups.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited.}
  \item Did you mention the license of the assets?
    \answerNo{All of the code, models, and datasets we used are publicly available.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We included our code and models in \supp.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{All the data is publicly available. }
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}



==> tables/ablate_shapenetpart.tex <==
\begin{wraptable}{r}{0.6\textwidth}
% \begin{table}[ht]
\centering
\small
\caption{\textbf{Additive study of sequentially applying training and model scaling strategies for object part segmentation on ShapeNetPart.} We use light \textcolor{green!50}{green}, \textcolor{blue!50}{purple}, \textcolor{yellow!60}{yellow}, and \textcolor{pink}{pink} background colors to denote data augmentation, optimization techniques, receptive field scaling, and model scaling, respectively.}
\label{tab:ablate_shapenetpart}
% \resizebox{1.0\textwidth}{!}{
\begin{tabular}{l|c|c}
\toprule
Improvements & Ins. mIoU (\%) & $\Delta$  \\
\midrule
PointNet++ & 85.1 & -- \\
% PointNet++ (best model selection) & $81.3\pm0.4$ & \textbf{+2.4} \\

% \rowcolor{green!5}
% $+$Normal Vector & $85.4$ & \textbf{+0.3} \\
\rowcolor{green!5}
$+$ Random rotation & $85.7\pm0.1$ & \textbf{+0.6} \\
\rowcolor{green!5}
$+$ Height appending & $86.0\pm0.1$ & \textbf{+0.3}\\
% \rowcolor{green!5}
% $-$ Jittering  & $86.0\pm0.0$ & \textbf{+0.0}\\  
\rowcolor{green!5}
$+$ Random scaling & $86.1\pm0.1$ & \textbf{+0.1}\\  
% \rowcolor{green!5}
% $+$ Feature drop &  & \textbf{+}\\  
\rowcolor{blue!5}
$+$ Training epochs $200\rightarrow400$ & $86.3\pm0.3$ & \textbf{+0.2} \\
\rowcolor{blue!5}
$+$ Adam $\rightarrow$ AdamW & $86.6\pm0.2$ & \textbf{+0.3} \\
\rowcolor{blue!5}
$+$ Step Decay $\rightarrow$ Cosine & $86.6\pm0.1$ & +0.0 \\

% \rowcolor{blue!5}
% \rowcolor{yellow!5}
% Normalize $\Delta_p$ (Equation \ref{eqn:pointnext_local_aggr})  & $86.7\pm0.3$ & \textbf{+0.3} \\
\midrule
\rowcolor{yellow!5}
$+$ Normalizing $\Delta_p$ &$86.7\pm0.0$&\textbf{+0.1} \\
\midrule
\rowcolor{red!5}
+ Scale down (PointNeXt-S (C=32))   & $86.5\pm0.0$ & \textbf{-0.2} \\
\rowcolor{red!5}
+ Scale up (PointNeXt-S (C=64))   & $86.9\pm0.1$ &  \textbf{+0.4} \\ 
% \rowcolor{red!5}
% + Scale up (PointNeXt-S (C=92))   &$87.1\pm0.1$ & \textbf{+0.2} \\
\rowcolor{red!5}
+ Scale up (PointNeXt-S (C=160))   &$87.2\pm0.0$ & \textbf{+0.3}\\
\bottomrule
\end{tabular}
% \end{table}
\end{wraptable}


==> tables/modelnet.tex <==
% % ModelNet Classification 
\begin{table}[ht]
\centering
\caption{\textbf{Shape classification on ModelNet40.} For PointNeXt, the average results without voting in three random runs are reported. $1024$ points without normals are used as input. Methods are in chronological order. PointNet++~\cite{qi2017pointnet2} (Ours) denotes PointNet++ trained with the improved strategies. }
\label{tab:modelnet40}
\resizebox{0.8\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{ l | c c | c c c}
\toprule
Method  & mAcc & OA & Params. & FLOPs & Throughput \\
\midrule
% 		3DShapeNets~\cite{wu2015modelnet}  & 77.3 & 84.7 \\
% 		VoxNet~\cite{maturana2015voxnet}  & 83.0 & 85.9 \\
% 		Subvolume~\cite{qi2016volumetric}  & 86.0 & 89.2 \\
% 		MVCNN~\cite{su15mvcnn}  & -- & 90.1 \\
% 		A-SCN~\cite{xie2018attentional}  & 87.6 & 90.0 \\
% 		Set Transformer~\cite{lee2019set}  & -- & 90.4 \\
% 		PAT~\cite{yang2019modeling}  & -- & 91.7 \\
% 		SpecGCN~\cite{wang2018local}  & -- & 92.1 \\
PointNet~\cite{qi2017pointnet} & 86.2 & 89.2 & 3.5 & 0.9 & 4212\\ % checked from PointNet
PointCNN~\cite{li2018pointcnn} & 88.1 & 92.2 & 0.6 & - & 44 \\ % checked from PointCNN
% 		PointWeb~\cite{zhao2019pointweb}  & 89.4 & 92.3 \\
% 		SpiderCNN~\cite{xu2018spidercnn}  & -- & 92.4 \\
PointConv~\cite{wu2019pointconv} & -- & 92.5 & - & - & -\\ % checked from pointConv
% 		Point2Sequence~\cite{liu2019point2sequence}  & 90.4 & 92.6 \\
% 		ShellNet~\cite{zhang2019shellnet} & - & 92.8 \\
KPConv~\cite{thomas2019kpconv} & - & 92.9 & - & - & - \\ % checked from KPConv
DGCNN~\cite{wang2019dgcnn} & 90.2 & 92.9 & 1.8 & 4.8 & 402 \\ % & 90.7 & 93.5 is 2048 points results 
DeepGCN \cite{li2021deepgcn}   & 90.9  & 93.6 & 2.2 & 3.9 & 263 \\ % the best from https://github.com/lightaime/deep_gcns_torch/blob/master/examples/modelnet_cls/README.md is  & 90.9  & 93.6
ASSANet-L ~\cite{qian2021assanet} & - & 92.9 &- &- & - \\ % checked from ASSA-Net
% 		InterpCNN~\cite{mao2019interpolated}  & -- & 93.0 \\
% 		Grid-GCN~\cite{xu2020grid} & 91.3 & 93.1\\
% 		PosPool~\cite{liu2020closer} & - & 93.2 \\
Point Cloud Transformer~\cite{guo2021pct} & - & 93.2 & -& - &- \\ % checked from PCT
Point Transformer~\cite{zhao2021pointtransformer} & 90.6 & 93.7 & -& - &- \\ % checked from transformer
% 		MVTN~\cite{hamdi2021mvtn} & 92.2 & 93.8 \\
% 		RPNet~\cite{ran2021learning} & - & 94.1 \\
CurveNet~\cite{xiang2021walk}  & - & 93.8 & - &- & - \\ % checked from CurveNet, also 1024 points,  94.2 with voting
PointMLP~\cite{ma2022pointmlp} $^\dagger$ & 90.9$\pm$0.4 & 93.7$\pm$0.2 & 13.2 & 31.3 & 191 \\ % ma: 91.4, oa: 94.5
\midrule
\gr  PointNet++~\cite{qi2017pointnet2} & - & 91.9& 1.5  & 1.7 & 1872 \\ % checked from pointConv
\gr  PointNet++~\cite{qi2017pointnet2} (Ours) &  $89.9\pm0.8$ & \reshll{$92.8\pm0.1$}{+}{0.9}	& 1.5 & 1.7 & 1872\\ % checked from pointConv
\gr \textbf{PointNeXt-S (ours)} & $90.8\pm0.2$ & \reshll{$93.2\pm0.1$}{+}{1.3} & 1.4 & 1.6 & 2040\\
\gr \textbf{PointNeXt-S (C=64)} & $90.9\pm0.5$ & \reshll{$93.7\pm0.3$}{+}{1.8} & 4.5 & 6.5 & 2033  \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item[$\dagger$] Average results in 6 runs without voting, reported in the official repository: \url{https://github.com/ma-xu/pointMLP-pytorch/issues/1}.  
\end{tablenotes}
\end{threeparttable}
}
\end{table}

==> tables/others.tex <==
% SemanticKITTI Segmentation 
% \subsubsection{Semantic KITTI} \cite{behley2019semantickitti} is a large scale 
% laser-based outdoor semantic segmentation dataset.
% There are 22 sequence in the odometry benchmark,
% while we split $00$ to $10$ as training set, and $11$ to $21$ as test set.
% Since we are interested in segmenting pointcloud from single scan,
% we adopt the setting of \textit{Semantic KITTI Single Scan Benchmark},
% resulting in a total number of 19 classes for training and evaluation.
%###############################################3
% \begin{table}[ht]
% {\Huge
% \centering
% \resizebox{1.0\columnwidth}{!}{
% \begin{tabular}{l|c |c| c| c| c| c| c |c |c| c| c| c| c| c| c| c| c| c| c| c}
% % \begin{tabular}{l|c c c c c c c c c c c c c c c c c c c c}

% \hline 
% Method & \begin{sideways} Mean IoU \end{sideways} 
% & \begin{sideways} Car \end{sideways} 
% & \begin{sideways} Bicycle \end{sideways} 
% & \begin{sideways} Motorcycle \end{sideways} 
% & \begin{sideways} Truck \end{sideways} 
% & \begin{sideways} Other-vehicle \end{sideways} 
% & \begin{sideways} Person \end{sideways} 
% & \begin{sideways} Bicyclist \end{sideways} 
% & \begin{sideways} Motorcyclist \end{sideways} 
% & \begin{sideways} Road \end{sideways} 
% & \begin{sideways} Parking \end{sideways} 
% & \begin{sideways} Sidewalk \end{sideways} 
% & \begin{sideways} Other-ground \end{sideways} 
% & \begin{sideways} Building \end{sideways} 
% & \begin{sideways} Fence \end{sideways} 
% & \begin{sideways} Vegetation \end{sideways} 
% & \begin{sideways} Trunk \end{sideways} 
% & \begin{sideways} Terrain \end{sideways} 
% & \begin{sideways} Pole \end{sideways} 
% & \begin{sideways} Traffic-sign \end{sideways}\\ 
% % & \begin{sideways} FPS (Hz) \end{sideways}  \\
% % \hline

% % \textbf{ClassRatio} &-&3.82 &0.02 &0.04 &0.18 &0.23 &0.04 &0.01 &0.01 &16.60 &1.19 &11.75 &0.44 &15.88 &6.97 &32.83 &0.68 &8.93 &0.31 &0.08 \\
% \hline
% PointNet \cite{qi2017pointnet}
% & 14.6 & 61.6 & 35.7 & 15.8 & 1.4 & 41.4 & 46.3 & 0.1 & 1.3 & 0.3 & 0.8 & 31.0 & 4.6 & 17.6 & 0.2 & 0.2 & 0.0 & 12.9 & 2.4  & 3.7 \\


% S-BKI \cite{gan2020bayesian} %correct
% & $51.3$ & $83.8$ & $30.6$ & $43.0$ & $26.0$ & $19.6$ & $8.5$ & $3.4$ & $0.0$ & $92.6$ & $65.3$ & $77.4$ & $30.1$ & $89.7$ & $63.7$ & $83.4$ & $64.3$ & $67.4$ & $58.6$ & $67.1$  \\
% RangeNet++ \cite{milioto2019rangenet++} %correct
% & $52.2$ & $91.4$ & $25.7$ & $34.4$ & $25.7$ & $23.0$ & $38.3$ & $38.8$ & $4.8$ & $91.8$ & $65.0$ & $75.2$ & $27.8$ & $87.4$ & $58.6$ & $80.5$ & $55.1$ & $64.6$ & $47.9$ & $55.9$  \\
% LatticeNet  \cite{rosu2019latticenet} %correct
% & $52.9$ & $92.9$ & $16.6$ & $22.2$ & $26.6$ & $21.4$ & $35.6$ & $43.0$ & $46.0$ & $90.0$ & $59.4$ & $74.1$ & $22.0$ & $88.2$ & $58.8$ & $81.7$ & $63.6$ & $63.1$ & $51.9$ & $48.4$ \\
% RandLA-Net \cite{hu2020randla} %correct
% & $53.9$ & $94.2$ & $26.0$ & $25.8$ & $40.1$ & $38.9$ & $49.2$ & $48.2$ & $7.2$ & $90.7$ & $60.3$ & $73.7$ & $20.4$ & $86.9$ & $56.3$ & $81.4$ & $61.3$ & $66.8$ & $49.2$ & $47.7$  \\
% PolarNet \cite{zhang2020polarnet} %correct
% & $54.3$ & $93.8$ & $40.3$ & $30.1$ & $22.9$ & $28.5$ & $43.2$ & $40.2$ & $5.6$ & $90.8$ & $61.7$ & $74.4$ & $21.7$ & $90.0$ & $61.3$ & $84.0$ & $65.5$ & $67.8$ & $51.8$ & $57.5$  \\
% MinkNet42 \cite{choy20194d} %correct
% & $54.3$ &  $94.3$ & $23.1$ & $26.2$ & $26.1$ & $36.7$ & $43.1$ & $36.4$ & $7.9$ & $91.1$ & $63.8$ & $69.7$ & $29.3$ & $92.7$ & $57.1$ & $83.7$ & $68.4$ & $64.7$ & $57.3$ & $60.1$ \\ %$3.4 HZ$
% 3D-MiniNet \cite{alonso2020MiniNet3D} %correct
% & $55.8$ & $90.5$ & $42.3$ & $42.1$ & $28.5$ & $29.4$ & $47.8$ & $44.1$ & $14.5$ & $91.6$ & $64.2$ & $74.5$ & $25.4$ & $89.4$ & $60.8$ & $82.8$ & $60.8$ & $66.7$ & $48.0$ & $56.6$ \\
% % SqueezeSegV3 \cite{xu2020squeezesegv3} %correct 
% % & $55.9$ & $92.5$ & $38.7$ & $36.5$ & $29.6$ & $33.0$ & $45.6$ & $46.2$ & $20.1$ & $91.7$ & $63.4$ & $74.8$ & $26.4$ & $89.0$ & $59.4$ & $82.0$ & $58.7$ & $65.4$ & $49.6$ & $58.9$ \\
% Kpconv \cite{thomas2019kpconv} %correct
% & $58.8$ & $96.0$ & $30.2$ & $42.5$ & $33.4$ & $44.3$ & $61.5$ & $61.6$ & $11.8$ & $88.8$ & $61.3$ & $72.7$ & $31.6$ & $90.5$ & $64.2$ & $84.8$ & $69.2$ & $69.1$ & $56.4$ & $47.4$ \\ 
% SalsaNext \cite{cortinhal2020salsanext}
% & $59.5$ & $91.9$ & $48.3$ & $38.6$ & $38.9$ & $31.9$ & $60.2$ & $59.0$ & $19.4$ & $91.7$ & $63.7$ & $75.8$ & $29.1$ & $90.2$ & $64.2$ & $81.8$ & $63.6$ & $66.5$ & $54.3$ & $62.1$    \\
% BAAF-Net~\cite{qiu2021semantic}
% & $59.9$ & $90.9$ & $74.4$ & $62.2$ & $23.6$ & $89.$ & $95.4$ & $48.7$ & $31.8$ & $35.5$ & $46.7$ & $82.7$ & $63.4$ & $67.9$ & $49.5$ & $55.7$ & $53.0$ & $60.8$ & $53.7$ & $52.0$ \\
% FusionNet   \cite{zhang2020deep}
% & $61.3$  & $95.3$ & $47.5$ & $37.7$ & $41.8$ & $34.5$ & $59.5$ & $56.8$ & $11.9$ & $91.8$ & $68.8$ & $77.1$ & $30.8$ & $92.5$ & $69.4$ & $84.5$ & $69.8$ & $68.5$ & $60.4$ & $66.5$\\
% % Cylinder3D  \cite{zhou2020cylinder3d}
% % & $61.8$ & $\textbf{96.1}$ & $54.2$ & $47.6$ & $38.6$ & $\textbf{45.0}$ & $65.1$ & $63.5$ & $13.6$ & $91.2$ & $62.2$ & $75.2$ & $18.7$ & $89.6$ & $61.6$ & $85.4$ & $69.7$ & $69.3$ & $\textbf{62.6}$ & $64.7$\\
% KPRNet    \cite{kochanov2020kprnet}
% & $63.1$ & $95.5$ & $54.1$ & $47.9$ & $23.6$ & $42.6$ & $65.9$ & $65.0$ & $16.5$ & $93.2$ & $73.9$ & $80.6$ & $30.2$ & $91.7$ & $68.4$ & $85.7$ & $69.8$ & $71.2$ & $58.7$ & $64.1$\\
% SPVNAS    \cite{tang2020searching}
% & $67.0$ & $97.2$ & $50.6$ & $50.4$ & $56.6$ & $58.0$ & $67.4$ & $67.1$ & $50.3$ & $90.2$ & $67.6$ & $75.4$ & $21.8$ & $91.6$ & $66.9$ & $86.1$ & $73.4$ & $71.0$ & $64.3$ & $67.3$\\
% % \cline{2-23} 
%  AF$^2$-S3Net \cite{cheng20212} 
% & $69.7$ & $94.5$ & $65.4$ & $86.8$ & $39.2$ & $41.1$ & $80.7$ & $80.4$ & $74.3$ & $91.3$ & $68.8$ & $72.5$ & $53.5$ & $87.9$ & $63.2$ & $70.2$ & $68.5$ & $53.7$ & $61.5$ & $71.0$ \\
% \hline
% PointNet++ & $47.16$ & $73.9$ & $28.6$ & $23.7$ & $34.0$ & $23.6$ & $5.8$ & $6.4$ & $3.6$ & $88.1$ & $56.3$ & $72.3$ & $24.2$ & $88.4$ & $60.7$ & $80.8$ & $62.8$ & $67.0$ & $50.3$ & $45.5$ \\

% \hline
% PointNet++~\cite{qi2017pointnet2} %correct
% & 20.1 & 72.0 & 41.8 & 18.7 & 5.6 & 62.3 & 53.7 & 0.9 & 1.9 & 0.2 & 0.2 & 46.5 & 13.8 & 30.0 & 0.9 & 1.0 & 0.0 &16.9 & 6.0 & 8.9 \\
% \gr \textbf{PointNeXt (ours)} & TBD \\

% \hline
% \end{tabular}}
% \caption{Segmentation IoU (\%) results on the SemanticKITTI test dataset.}
% \label{bigtable}}
% \end{table} 


% \begin{table}[ht]
% \tablestyle{5.0pt}{1.02}
% \footnotesize
% \resizebox{1.0\columnwidth}{!}{
% \begin{tabular}{ll|cccc}
% % \begin{tabular}{@{\hskip -0.05ex}l|c@{\hskip 1ex}c|c@{\hskip 1ex}c|c@{\hskip 1ex}c|c@{\hskip 1ex}c}

% % & \cnn{}-T/S/B/L & \cnn{}-T/S/B/L/XL \\
% % \multirow{2}{*}{(pre-)training config} & ImageNet-1K & ImageNet-22K \\
% % & 224$^2$ & 224$^2$ \\
% \hline
%  & Dataset & ScanObjectNN & S3DIS  & SemanticKITTI \\
% \midrule
% \multicolumn{2}{c|}{data augmentation}
%  & - & - & - & \\
% \midrule
% % training strategies
% \multirow{6}{4em}{training strategies} 
% & optimizer & AdamW & AdamW & AdamW \\
% &weight decay & 0.05 & 0.05 & 1.0e-4 \\
% &optimizer momentum & $\beta_1, \beta_2{=}0.9, 0.999$ & $\beta_1, \beta_2{=}0.9, 0.999$ & $\beta_1, \beta_2{=}0.9, 0.999$ \\
% &learning rate schedule & cosine decay & cosine decay& cosine decay \\
% &base learning rate & 4e-3 & 4e-3 & 2e-3\\
% &training epochs & 300 & 90 & 40 \\
% \midrule 
% \multirow{3}{4em}{receptive field} &radius &  None?& 2.0 & 2.0 &  \\ 
% & kernel size & None? & None? &None? &  \\ 
% & normalized neighbors & None? & None? &None? & \\

% \midrule 
% number of stages && None? & None?&None?   \\ 
% separable downsampling layer & & None?& None?&None?  \\ 
% residual connection  & & None? & None? & None?  \\ 
% \midrule
% \end{tabular}}
% \caption{Training settings on three datasets}
% \label{tab:train_detail}
% \end{table}


% PartNet Segmentation. 
% \begin{table}[htb!]
% \resizebox{1.0\columnwidth}{!}{
% \begin{tabular}{l|ccccccccccccccccccc}
% \hline
% Method 
% &\begin{sideways}mioU \end{sideways}
% & \begin{sideways}bed \end{sideways}
% &  \begin{sideways}bottle\end{sideways}
% & \begin{sideways} chair \end{sideways}
% & \begin{sideways} clock \end{sideways}
% &  \begin{sideways}dish-washer \end{sideways}
% &  \begin{sideways}display \end{sideways}
% &  \begin{sideways}door \end{sideways}
% &  \begin{sideways}ear-phone \end{sideways}
% &\begin{sideways}faucet \end{sideways}
% &  \begin{sideways}knife \end{sideways}
% &  \begin{sideways}lamp\end{sideways}
% & \begin{sideways} microwave\end{sideways}
% &  \begin{sideways}refrigerator\end{sideways}
% & \begin{sideways} storage \end{sideways}
% & \begin{sideways} table \end{sideways}
% & \begin{sideways} trash can \end{sideways}
% &  \begin{sideways}vase \end{sideways}\\
%   \hline
% PointNet~\cite{qi2017pointnet}   & 35.6 & 13.4 & 29.5 & 27.8 & 28.4 & 48.9 & 76.5 & 30.4 & 33.4 & 47.6 & 32.9 & 18.9 & 37.2 & 33.5 & 38.0 & 29.0 & 34.8 & 44.4 \\
% PointNet++\cite{qi2017pointnet2} & 42.5 & 30.3 & 41.4 & 39.2 & 41.6 & 50.1 & 80.7 & 32.6 & 38.4 & 52.4 & 34.1 & 25.3 & 48.5 & 36.4 & 40.5 & 33.9 & 46.7 & 49.8 \\
% PointCNN~\cite{li2018pointcnn}  & 46.5 & 41.9 & 41.8 & 43.9 & 36.3 & 58.7 & 82.5 & 37.8 & 48.9 & 60.5 & 34.1 & 20.l & 58.2 & 42.9 & 49.4 & 21.3 & 53.l & 58.9 \\
% DGCNN~\cite{wang2019dgcnn}      & 44.6 & 36.1 & 48.9 & 40.7 & 34.4 & 55.9 & 80.4 & 30.8 & 45.1 & 51.5 & 42.9 & 22.6 & 50.9 & 33.6 & 46.9 & 34.2 & 50.6 & 53.4 \\
% DeepGCN~\cite{li2021deepgcn}  & 45.1 & 35.9 & 49.3 & 41.1 & 33.8 & 56.2 & 81.0 & 31.1 & 45.8 & 52.8 & 44.5 & 23.1 & 51.8 & 34.9 & 47.2 & 33.6 & 50.8 & 54.2 \\
% ADConvnet~\cite{wong2020efficient}  & 47.0 & 42.l & 41.7 & 44.2 & 35.9 & 58.4 & 82.9 & 38.1 & 48.5 & 58.9 & 33.3& 19.8 & 58.4 & 43.4 & 49.2 & 34.2 & 52.9 & 57.5 \\
% PHGCN   ~\cite{wong2021persistent}            & 49.8 & 43.0 & 48.7 & 45.9 & 41.9 & 59.3 & 84.2 & 37.5 & 50.2 & 62.9 & 46.1 & 26.2 & 59.1 & 44.2 & 49.1 & 35.2 & 54.3 & 59.5 \\
% \hline
% \end{tabular}}
% \caption{Results on the PartNet dataset.}
% \end{table}

% \begin{table}[ht]
% 	\centering
% 	\begin{tabular}{ l | c c}
% 		Method & val & test \\
% 		\hline
% % 		PointNet~\cite{qi2017pointnet} & - & - \\
% % 		PointNet++~\cite{qi2017pointnet2} &- &- \\
% 		PointCNN~\cite{li2018pointcnn} & - & 46.5 \\
% % 		DGCNN~\cite{wang2019dgcnn}  & - & - \\
% 		DeepGCN & - & 45.1 \\
% % 		ShellNet~\cite{zhang2019shellnet}  & - & - \\	
% % 		KPConv~\cite{thomas2019kpconv}  & - & - \\
% % 		Grid-GCN & - & - \\
% % 		PVCNN  & - & -\\
% % 		ASSANet(L)  & - & - \\
% 		PosPool  & 50.6 & 53.8 \\
% %         CurveNet  & - & - \\
% % 		PointTransformer & - & - \\
% % 		Point Cloud Transformer  & - & -  \\

	
% 	\end{tabular}
% 	\caption{Results on the PartNet dataset.}
% 	\label{tab:partnet}
% 	\vspace{-2mm}
% \end{table}




% ScanNet Segmentation
% \begin{table}[t]
% 	\centering
% 	\begin{tabular}{ l | c c}
% 		Method & OA & latency(ms) \\
% 		\hline
		
% 		PointNet~\cite{qi2017pointnet}  & 73.9 & 20.3 \\
% 		PointNet++~\cite{qi2017pointnet2}  & 84.5 & 72.3 \\ % from shellnet
% 		PointCNN~\cite{li2018pointcnn}  & 85.1 & 250 \\ % from Grid-GCN ??
% 		DGCNN~\cite{wang2019dgcnn}  & - & - \\
% 		DeepGCN & - & - \\
% 		ShellNet~\cite{zhang2019shellnet}  & 85.2 & - \\
% 		KPConv~\cite{thomas2019kpconv}  & - & - \\ % 68.6 ???
% 		Grid-GCN & 85.4 & 7.48 \\
% 		PVCNN  & - & -\\
% 		ASSANet(L)  & - & - \\
% 		PosPool  & - & - \\
%         CurveNet  & - & - \\
% 		PointTransformer & - & - \\
% 		Point Cloud Transformer  & - & -  \\
% 	\end{tabular}
% 	\caption{Results on the ScanNet dataset.}
% 	\label{tab:scannet}
% 	\vspace{-2mm}
% \end{table}



% \begin{table*}[ht]
% \setlength{\tabcolsep}{2.5pt}
% \small\centering
% \begin{tabular}{lccccccccccc}
%     % \toprule
%      & \multicolumn{3}{c}{Car} & \multicolumn{3}{c}{Pedestrian} & \multicolumn{3}{c}{Cyclist} \\
%     % \cmidrule(lr){2-3}\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}
%      & Easy & Mod. & Hard & Easy & Mod. & Hard & Easy & Mod. & Hard \\
%   \hline
%     F-PointNet~ & 83.26 & 69.28 & 62.56 & 65.08 & 55.85 & 49.28 & 74.54 & 55.95 & 52.65 \\
%     F-PointNet++~   & 83.76 & 70.92 & 63.65 & 70.00 & 61.32 & 53.59 & 77.15 & 56.49 & 53.37 \\
%     \hline
%     PointNet~\cite{qi2017pointnet} & - & - \\
% 	PointNet++~\cite{qi2017pointnet2} &- &- \\
%     PointCNN~\cite{li2018pointcnn} & - & - \\
%     DGCNN~\cite{wang2019dgcnn}  & - & - \\
%     DeepGCN & - & - \\
%     ShellNet~\cite{zhang2019shellnet}  & - & - \\	
%     KPConv~\cite{thomas2019kpconv}  & - & - \\
%     Grid-GCN & - & - \\
%     PVCNN  & 84.02 & \textbf{71.54} & \textbf{63.81} & \textbf{73.20} & \textbf{64.71} & \textbf{56.78} & \textbf{81.40} & \textbf{59.97} & \textbf{56.24} \\
%     ASSANet(L)  & - & - \\
% 	PosPool  & - & - \\
%     CurveNet  & - & - \\
%     PointTransformer & - & - \\
% 	Point Cloud Transformer  & - & -  \\
		
   
% \end{tabular}
% \caption{Results of 3D object detection on the \emph{val} set of KITTI. }
% \label{tab:kitti_results}
% \vspace{-10pt}
% \end{table*}


% \begin{table}[ht]
% 	\centering
% 	\begin{tabular}{ l | c c}
% 		Method & metrics1 & metrics2 \\
% 		\hline
% 		PointNet~\cite{qi2017pointnet} & 14.6 & - \\
% 		PointNet++~\cite{qi2017pointnet2} &20.1 &- \\
% % 		PointCNN~\cite{li2018pointcnn} & - & - \\
% % 		DGCNN~\cite{wang2019dgcnn}  & - & - \\
% % 		DeepGCN & - & - \\
%         % ShellNet~\cite{zhang2019shellnet}  & - & - \\		
% 		KPConv~\cite{thomas2019kpconv}  & 58.8 & - \\
% % 		Grid-GCN & - & - \\
% % 		PVCNN  & - & -\\
% % 		ASSANet(L)  & - & - \\
% % 		PosPool  & - & - \\
% %         CurveNet  & - & - \\
% %         PointTransformer & - & - \\
% % 		Point Cloud Transformer  & - & -  \\
% 	\end{tabular}
% 	\caption{Results on the SemanticKITTI dataset.}
% 	\label{tab:kitti}
% 	\vspace{-2mm}
% \end{table}


% ModelNet
% \begin{table}[]
% \small
%     \centering
    
%  \vspace{1mm}
%     \begin{tabular}{l|ccc|ccc}
%     \toprule
%          Method& Inputs & mAcc(\%) &OA(\%) & Param. &\makecell{ Train\\speed} &\makecell{ Test\\speed} \\
%          \midrule
%          PointNet~\cite{qi2017pointnet}   & 1k P &86.0 &89.2 & & & \\
%         %  A-SCN~\cite{xie2018attentional}      & 1k P&-&89.8  & & & \\
%         %  SO-Net~\cite{li2018so}     &2k P+N &-&90.9  & & & \\
%         %  Kd-Net~\cite{klokov2017escape}     & 32k P &-&91.8  & & & \\
%          PointNet++~\cite{qi2017pointnet2} & 1k P &-&90.7  & 1.41M&\textbf{223.8} &\textbf{308.5} \\
%          PointNet++~\cite{qi2017pointnet2} &5k P+N &-&91.9  & 1.41M& & \\
%          \midrule
%          PointCNN~\cite{li2018pointcnn}   &1k P &88.1&92.5  & & & \\
%         %  PointGrid~\cite{le2018pointgrid}  &1k P &-&92.0  & & & \\
%         %  PCNN~\cite{atzmon2018point}       &1k P&-&92.3  & & & \\
%         %  PointWeb~\cite{zhao2019pointweb}   &1k P &-&92.3  & & & \\
         
%          PointConv~\cite{wu2019pointconv}  &1k P+N &-&92.5  &18.6M &17.9 &10.2 \\
%         %  A-CNN~\cite{komarichev2019cnn}      &1k P+N &-&92.6  & & & \\
%         %  P2Sequence~\cite{liu2019point2sequence} & 1k P &-&92.6  & & & \\
%          KPConv~\cite{thomas2019kpconv}     & 7k P &-&92.9  &15.2M &31.0* &80.0* \\
%          DGCNN~\cite{wang2019dgcnn}      & 1k P &90.2&92.9  & & &  \\
%          RS-CNN~\cite{liu2019relation}     & 1k P &-&92.9  & & & \\
%          DensePoint~\cite{liu2019densepoint} &1k P &-&93.2  & & & \\
%         %  InterpCNN~\cite{mao2019interpolated}  &1k P &-&93.0  & & & \\
%          PointASNL~\cite{yan2020pointasnl}  & 1k P &-&92.9  & & & \\
%          PosPool~\cite{liu2020closer}    &5k P &-&93.2  & & & \\
%         %  FPConv~\cite{lin2020fpconv}     & 1k P & &92.5 & & & \\
%         %  Grid-GCN~\cite{xu2020grid}   & 1k P &-&93.1  & & & \\
%         %  Point2Node~\cite{han2020point2node} &1k P &-&93.0  & & & \\
%          Point Transformer~\cite{engel2020point}  &1k P &-&92.8  & & & \\
%          GBNet~\cite{qiu2021geometric} &1k P &\textcolor{blue}{91.0} &93.8 &8.39M &16.3 &112 \\
%          GDANet~\cite{xu2021learning}& 1k P &-&93.8  &\textcolor{blue}{0.93M} &26.3 & 14.0\\
%         %  PA-PointNet~\cite{xu2021paconv}   & 1k P &-&93.2  & & & \\
%          PA-DGC~\cite{xu2021paconv}    &1k P &-&93.9  & & & \\
%          MLMSPT~\cite{han2021point}  &1k P &-&92.9  & & & \\
         
%          PCT~\cite{guo2021pct}        &1k P &-&93.2  & & & \\
%          Point Trans.~\cite{zhao2021pointtransformer}  &1k P &90.6&93.7  & & & \\
%         %  93.8 94.2
%         CurveNet~\cite{xiang2021walk} &1k P &-&\textcolor{blue}{94.2}  &2.04M & 20.8&15.0 \\
%         %  \midrule
%          %PointMLP &1k P &\textbf{91.3} &\textbf{93.8}  & & & \\ 
%          %model31A-20210818204651
%         %  PointMLP &1k P &91.2 &93.8  & & & \\  %model31A-20210818145058
        
%         %  %94.044 mean_acc: 91.299 see /scratch/ma.xu1/pointsMLP/classification/checkpoints/model31A-20210818204651/evaluate_voting-20210823142104seed_8709.log
%         % PointMLP {\small \textbf{w/ vot.} (previous version)} &1k P &\textbf{91.3} &\textbf{94.0}  & & & \\  %model31A-20210818145058
        
%         % evaluate_voting-20210828170909seed_6276.log all_acc: 94.084 mean_acc: 91.286
%         %PointMLP {\small \textbf{w/ vot.}} &1k P &\textbf{91.3} &\textbf{94.1}  & & & \\  %model31A-20210818145058
        
        
%         % model31C-20210829112651 Best Test acc_B: 90.766/Best Test acc: 93.72
%         %evaluate_voting-20210831024947seed_3319.log all_acc: 94.165 mean_acc: 91.12
%         % PointMLP &1k P &90.8 &93.7  & & & \\ %model31C-20210829112651
%         % PointMLP {\small \textbf{w/ vot.}} &1k P &\textbf{91.1} &\textbf{94.2}  & & & \\  %evaluate_voting-20210831024947seed_3319.log
        
        
%         % PointMLP {\small \textbf{w/o vot.}}&1k P &91.3 &94.1  &12.6M &47.1 &112 \\ %model31C-20210905101714
%         PointMLP  &1k P &\textbf{91.4} &\textbf{94.5}  &12.6M &47.1 &112\\ 
%         %modelelite3X10-20211002174353
%         %modelelite3X10-20211002203755 also same
%         % PointMLP-elite {\small \textbf{w/o vot.}} &1k P &90.9 &93.6  &\textbf{0.68M} &\textcolor{blue}{116} &\textcolor{blue}{176} \\
%         % %modelelite3X10-20211002203755/evaluate_voting-20211004083506seed_742.log
%         % PointMLP-elite {\small \textbf{w/ vot.}} &1k P &90.7 & 94.0 &\textbf{0.68M} &\textcolor{blue}{116} &\textcolor{blue}{176} \\ 
        
%          \bottomrule
%     \end{tabular}
%     \caption{Classification results on ModelNet40 dataset. }
%     % PointMLP is able to achieve the best performance on both mean class accuracy (mAcc) and overall accuracy (OA). }
%     \label{tab:classification-modelnet40}
% \end{table}



% \begin{table}
% \centering
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{l|ccccccccccccccccc} 
% \hline            
% Method          
% & \begin{sideways}mioU \end{sideways}
% & \begin{sideways}airplane \end{sideways}
% & \begin{sideways}bag  \end{sideways}
% & \begin{sideways}cap  \end{sideways}
% & \begin{sideways}car  \end{sideways}
% & \begin{sideways}chair \end{sideways}
% & \begin{sideways}ear phone \end{sideways}
% & \begin{sideways}guitar \end{sideways}
% &\begin{sideways} knife \end{sideways}
% & \begin{sideways}lamp \end{sideways}
% & \begin{sideways}laptop \end{sideways}
% & \begin{sideways}motor \end{sideways}
% & \begin{sideways}mug  \end{sideways}
% & \begin{sideways}pistol\end{sideways}
% & \begin{sideways}rocket \end{sideways}
% & \begin{sideways}skateboard \end{sideways}
% & \begin{sideways}table \end{sideways} \\ 
% \hline
% PointNet~\cite{qi2017pointnet}    & 83.7 & 83.4     & 78.7 & 82.5 & 74.9 & 89.6  & 73.0      & 91.5   & 85.9  & 80.8 & 95.3   & 65.2  & 93.0 & 81.2   & 57.9   & 72.8        & 80.6   \\ 
% PointNet++~\cite{qi2017pointnet2} & 85.1 & 82.4     & 79.0 & 87.7 & 77.3 & 90.8  & 71.8      & 91.0   & 85.9  & 83.7 & 95.3   & 71.6  & 94.1 & 81.3   & 58.7   & 76.4        & 82.6   \\ 
% \hline
% SPLATNet~\cite{su2018splatnet}   & 85.4 & 83.2     & 84.3 & 89.1 & 80.3 & 90.7  & 75.5      & 92.1   & 87.1  & 83.9 & 96.3   & 75.6  & 95.8 & 83.8   & 64.0   & 75.5        & 81.8   \\ 
% PointCNN~\cite{li2018pointcnn}  & 86.1 & 84.1     & 86.4 & 86.0 & 80.8 & 90.6  & 79.7      & 92.3   & 88.4  & 85.3 & 96.1   & 77.2  & 95.3 & 84.2   & 64.2   & 80.0        & 83.0   \\ 
% DGCNN ~\cite{wang2019dgcnn}      & 85.0 & 84.0     & 83.4 & 86.7 & 77.8 & 90.6  & 74.7      & 91.2   & 87.5  & 82.8 & 95.7   & 66.3  & 94.9 & 81.1   & 63.5   & 74.5        & 82.6   \\ 
% DeepGCN~\cite{li2021deepgcn}   & 85.5 & 85.3     & 83.5 & 86.6 & 78.1 & 90.9  & 75.1      & 91.5   & 86.8  & 83.1 & 95.9   & 68.1  & 95.2 & 80.9   & 63.8   & 74.8        & 83.1   \\ 
% PartNet~\cite{mo2019partnet}    & 87.4 & 87.8     & 86.7 & 89.7 & 80.5 & 91.9  & 75.7      & 91.8   & 85.9  & 83.6 & 97.0   & 74.6  & 97.3 & 83.6   & 64.6   & 78.4        & 85.8   \\ 
% ADConvnet~\cite{wong2020efficient}  & 87.0 & 87.4     & 86.4 & 89.5 & 80.1 & 91.4  & 78.9      & 91.5   & 86.2  & 82.9 & 96.9   & 76.9  & 97.1 & 84.0   & 64.3   & 79.6        & 85.4   \\ 
% PHGCN~\cite{wong2021persistent}  & 89.2 & 88.9     & 86.6 & 90.2 & 81.5 & 92.8  & 80.2      & 93.1   & 88.2  & 87.8 & 97.5   & 79.2  & 98.6 & 85.8   & 64.7   & 80.9        & 87.8   \\
% \hline
% \end{tabular}}
% \caption{Object part segmentation results on the ShapeNetPart dataset.}
% \end{table}


==> tables/roadmap.tex <==
% \begin{wraptable}{r}{0.5\textwidth}
\begin{table}[t]
% \tablestyle{5.0pt}{1.02}
% \footnotesize
\caption{Performance gains by the improved training and model scaling strategies on the ScanObjectNN object classification \cite{uy-scanobjectnn-iccv19} and the S3DIS semantic segmentation \cite{armeni2016s3dis}. }
\label{tab:roadmap_scaobjectnn}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{ll|ccc|ccc}
\specialrule{1.25pt}{0pt}{1pt}
 & \textbf{Roadmap} &  ScanObjectNN~\cite{uy-scanobjectnn-iccv19} & OA (\%) & GFLOPs & S3DIS~\cite{armeni2016s3dis} & mIoU (\%) & GFLOPs\\
\midrule
\textbf{Baseline} & PointNet++ \cite{qi2017pointnet2} & -  & 77.9 & 1.71 & - & & 28.96 \\
\midrule
\multirow{2}{6em}{\textbf{training strategies}}
& data augmentation & refer to Table \ref{tab:train_tech} & $82.7\pm0.3$ & 1.71& \\
& optimization & refer to Table \ref{tab:train_tech} & $85.7\pm1.3$ & 1.71 & \\
\midrule
\multirow{2}{6em}{\textbf{Receptive Field}}
& radius & $\{0.2, 0.4\} \rightarrow \{0.15, 0.3\}$ & $86.1\pm0.1$ & 1.71\\
& normalize $\Delta_p$ & refer to Equation \ref{eqn:pointnext_local_aggr}  & $86.4\pm0.4$ & 1.71 \\ 
& kernel size & $\{32, 64\} \rightarrow \{32, 32\}$  & $86.5\pm0.2$ & 1.16 & \\
\midrule
% \multirow{2}{6em}{\textbf{ResNetify}}
% & 4 stages & $\{64, 128\} \rightarrow \{32, 64, 128, 256\}$  & $86.7\pm0.3$  & 1.71 & - & - \\
% & stem MLP & - & & 1.71 &  - & \\
% & residual connection &  - & $87.7\pm0.4$ & 1.64  & - &  \\
% \midrule
% \textbf{Inverted MLP}
% & - &  -  & \GQ{exp}  & - &  \\
% \midrule
\multirow{2}{6em}{\textbf{Model Scaling}}
& depth scaling &  -  & \GQ{exp}  & - &  \\
& stage ratio &  -  & \GQ{exp}  & - &  \\
& With scaling &  -  & \GQ{exp}  & - &  \\
\bottomrule
\end{tabular}}
\end{table}


==> tables/s3dis_allarea.tex <==
\begin{wraptable}{b}{0.75\textwidth}
\vspace{-1.3em}
\small
\centering
\caption{\textbf{Semantic segmentation on S3DIS with 6-fold cross-validation.} The improvements of our PointNeXt over PointNet++~\cite{qi2017pointnet2} are highlighted in \hl{green} color. Methods are in chronological order.}
\label{tab:s3dis_6fold}
\vspace{-0.5em}
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{ l | l l l |c c c}
\toprule
\textbf{Method} & mIoU & OA & mAcc  & Params.  & FLOPs  & Throughput\\ 
 & (\%) & (\%) & (\%) & M  & G & (ins./sec.) \\ % & G
\midrule
PointNet~\cite{qi2017pointnet} & 47.6 & 78.5 & 66.2  & 3.6 & 35.5 & 162 \\ % from point cnn on all areas
PointCNN~\cite{li2018pointcnn}& 65.4 & 88.1 & 75.6  & 0.6 & - & -\\ % confirmed on the sup material on PointCNN
DGCNN~\cite{wang2019dgcnn}  & 56.1 & 84.1 & -  & 1.3 & - & 8 \\  % 6 folds on all areas from PCT
% RSNet~\cite{huang2018rsnet} & -- & 66.5 & 56.5 & - & - & - \\ % 6 folds from RS-Net sup material, oa-macc-miou
DeepGCN~\cite{li2019deepgcns} & 60.0  & 85.9 & -& 3.6 & - & 3 \\ % confirmed on all areas from Deep-GCN main table
% SPGraph~\cite{landrieu2018spg} & 85.5 & 73.0 & 62.1 & - & - & -\\ % confirmed on all areas from SPGraph, oa-macc-miou
% PAT~\cite{yang2019modeling} & -- & 76.5 & 64.3 & - & - & -\\ % confirmed on all areas from PAT, oa-macc-miou
% PointWeb~\cite{zhao2019pointweb} & 87.3 & 76.2 & 66.7& - & - & - \\ % confirmed on PointWeb all areas, oa-macc-miou
% ShellNet~\cite{zhang2019shellnet} & 66.8 & 87.1 & - & - & - & - \\ % confirmed on all areas
KPConv~\cite{thomas2019kpconv} & 70.6 & - & 79.1  & 15.0 & - & 30  \\ % confirmed on all throughput 1 areas from KPconv and randlenet In open3dml paras =18.3
RandLA-Net~\cite{hu2020randla} & 70.0 & 88.0 & 82.0  & 1.3  & 5.8 & 159 \\ % confirmed on all areas from randlenet throughput Throughput (ins./s): 14.447360277710908  5.76    2.84    1.300
% SCF-Net~\cite{fan2021scf} & 88.4 & 82.7 & 71.6 \\ %  scf net , corrected from SCF-Net confirmed on all areas, oa-macc-miou
BAAF-Net~\cite{qiu2021baaf} & 72.2 & 88.9 & \textbf{83.1}  & 5.0 & - & 10 \\ % confirmed on all areas from BAAF-Net
Point Transformer~\cite{zhao2021pointtransformer} & 73.5 & 90.2 & 81.9 & 7.8 & 5.6  & 34 \\ % confirmed on all areas from Transformer, flops=& 5.64
CBL~\cite{Tang2022ContrastiveBL} & 73.1 & 89.6 & 79.4 & 18.6  &- & -\\ %18628861
% RepSurf-U~\cite{ran2022surface} & 90.9 & 82.6 & 74.3 & 0.976 & -\\, oa-macc-miou
\midrule
\gr
PointNet++~\cite{qi2017pointnet2}	 &  54.5 & 81.0 & 67.1 & 1.0 & 7.2 & 186 \\ % from point cnn,
\gr
\textbf{PointNeXt-S (ours)} & \reshll{68.0}{+}{13.5} & \reshll{87.4}{+}{6.4} & \reshll{77.3}{+}{10.2} & 0.8  & 3.6 & \textbf{227} \\
\gr
\textbf{PointNeXt-B (ours)} & \reshll{71.5}{+}{17.0} & \reshll{88.8}{+}{7.8} & \reshll{80.2}{+}{13.1} & 3.8 & 8.9  & 158\\
\gr
\textbf{PointNeXt-L (ours)} & \reshll{73.9}{+}{19.4}  & \reshll{89.8}{+}{8.8} &  \reshll{82.2}{+}{15.1}& 7.1 & 15.2  & 115 \\
\gr
\textbf{PointNeXt-XL (ours)} & \reshl{\textbf{74.9}}{+}{20.4}  & \reshl{\textbf{90.3}}{+}{9.3} & \reshll{83.0}{+}{15.9}& 41.6 & 84.8 & 46 \\ % flops=& 89.64
\bottomrule[1pt]
\end{tabular}}
\end{wraptable}

==> tables/s3dis_area5.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Semantic segmentation results on S3DIS area 5.} The mean$\pm$std (OA, mACC, and mIoU) and the average IoU per class of three random runs are reported. }
\label{tab:s3dis_area5}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ l | c c c | c c c c c c c c c c c c c}
\toprule[1pt]
\textbf{Method}
&\begin{sideways}   OA   \end{sideways}
&\begin{sideways}   mAcc \end{sideways}
&\begin{sideways}   mIoU \end{sideways}
&\begin{sideways}   ceiling \end{sideways}
&\begin{sideways}   floor \end{sideways}
&\begin{sideways}   wall \end{sideways}
&\begin{sideways}   beam \end{sideways}
&\begin{sideways}   column\end{sideways}
&\begin{sideways}   window \end{sideways}
&\begin{sideways}   door \end{sideways}
&\begin{sideways}   table \end{sideways}
&\begin{sideways}   chair \end{sideways}
&\begin{sideways}   sofa \end{sideways}
&\begin{sideways}   bookcase \end{sideways}
&\begin{sideways}   board \end{sideways}
&\begin{sideways}   clutter\end{sideways} \\
\midrule
PointNet~\cite{qi2017pointnet} & - & 49.0 & 41.1 & 88.8 & 97.3 & 69.8 & 0.1 & 3.9 & 46.3 & 10.8 & 59.0 & 52.6 & 5.9 & 40.3 & 26.4 & 33.2\\ % from pointcnn
% PointNet~\cite{qi2017pointnet}& 78.5& 66.2 &47.6& 88.0 &88.7 &69.3 &42.4 &23.1& 47.5 &51.6& 54.1& 42.0 &9.6& 38.2 &29.4 &35.2 \\% this row is on all areas from pointcnn

% SegCloud~\cite{tchapmi2017segcloud} & -- & 57.4 & 48.9 & 90.1 & 96.1 & 69.9 & 0.0 & 18.4 & 38.4 & 23.1 & 70.4 & 75.9 & 40.9 & 58.4 & 13.0 & 41.6\\

% TangentConv~\cite{tatarchenko2018tangent} & -- & 62.2 & 52.6 & 90.5 & 97.7 & 74.0 & 0.0 & 20.7 & 39.0 & 31.3 & 77.5 & 69.4 & 57.3 & 38.5 & 48.8 & 39.8 \\

% DGCNN~\cite{wang2019dgcnn} & 82.3 & 58.7 & 50.0 &\WM{This row is on area 5 from github }\\ % from PCT, from https://github.com/AnTao97/dgcnn.pytorch/issues/20 Test :: test area: 5, test acc: 0.823081, test avg acc: 0.586665, test iou: 0.499677

PointCNN~\cite{li2018pointcnn} & 85.9 & 63.9 & 57.3  & 92.3 & 98.2 & 79.4 & 0.0 & 17.6 & 22.8 & 62.1 & 74.4 & 80.6 & 31.7 & 66.7 & 62.1 & 56.7\\ % \WM{This row is on area5 see arixv their supple material }

DGCNN~\cite{wang2019dgcnn} & 83.6 & - & 47.9 & - & - & - & - & - & - & - & - & - & - & - & - & - \\ % \WM{This row is on area 5  from PVCNN reported}

% 			SPGraph~\cite{landrieu2018spg} & 86.4 & 66.5 & 58.0 & 89.4 & 96.9 & 78.1 & 0.0 & 42.8 & 48.9 & 61.6 & 84.7 & 75.4 & 69.8 & 52.6 & 2.1 & 52.2\\
% 			PCCN~\cite{wang2018pccn} & -- & 67.0 & 58.3 & 92.3 & 96.2 & 75.9 & 0.3 & 6.0 & 69.5 & 63.5 & 66.9 & 65.6 & 47.3 & 68.9 & 59.1 & 46.2\\
% 			PAT~\cite{yang2019modeling} & -- & 70.8 & 60.1 & 93.0 & 98.5 & 72.3 & 1.0 & 41.5 & 85.1 & 38.2 & 57.7 & 83.6 & 48.1 & 67.0 & 61.3 & 33.6\\
% PointWeb~\cite{zhao2019pointweb} & 87.0 & 66.6 & 60.3 & 92.0 & 98.5 & 79.4 & 0.0 & 21.1 & 59.7 & 34.8 & 76.3 & 88.3 & 46.9 & 69.3 & 64.9 & 52.5 \\
% 			HPEIN~\cite{jiang2019hpein} & 87.2 & 68.3 & 61.9 & 91.5 & 98.2 & 81.4 & 0.0 & 23.3 & 65.3 & 40.0 & 75.5 & 87.7 & 58.5 & 67.8 & 65.6 & 49.4 \\
% 			MinkowskiNet~\cite{thomas2019kpconv} & -- & 71.7 & 65.4 & 91.8 & 98.7 & 86.2 & 0.0 & 34.1 & 48.9 & 62.4 & 81.6 & 89.8 & 47.2 & 74.9 & 74.4 & 58.6 \\
% RSNet~\cite{huang2018recurrent}  & -& 59.4& 51.9& 93.3& 98.4 &79.2 &0.0 &15.8& 45.4 &50.1 &65.5& 67.9 &22.5& 52.5& 41.0 &43.6 \\% not sure their result is at area 5

DeepGCN~\cite{li2019deepgcns} & - & - & 52.5 & - & - & - & - & - & - & - & - & - & - & - & - & -   \\ % from deepGCN ablation study

% Grid-GCN~\cite{xu2020grid} & 86.9 & - & 57.8& 94.1 &97.3  &77.7 &0.0 &16.6 &32.9& 58.5& 72.2& 81.3 &36.5 &68.7 &64.5 &50.5 \\ % from ASSA-Net, and Grid-GCN,this one must be in area5 confirmed



% SPGraph: oa : 86.38 macc: 66.50 miou: 58.04
% PAT : miou : 60.07
% PointWeb : 86.97 66.64 60.28 

% PVCNN~\cite{liu2019point} & - & 82.6 & 46.9 \\ % from PVCNN, based on 8*4096 points, same as pointnet
PVCNN~\cite{liu2019pvcnn} & 87.1  & - & 59.0 & - & - & - & - & - & - & - & - & - & - & - & - & - \\ % from PVCNN, based on 4*8192 points, 
% RandLA-Net~\cite{thomas2019kpconv} &  - & - & 62.5 &  \\% They don't report area5 on paper, this is from https://github.com/QingyongHu/RandLA-Net/issues/84 5 ---- 62.51 
% PCTransformer~\cite{guo2021pct} &-& 67.7 & 61.3 & 92.5 & 98.4 & 80.6 & 0.0 & 19.4 & 61.6 & 48.0 & 76.6 & 85.2& 46.2& 67.7& 67.9& 52.3 \\ % from PCT verified at area 5

% PosPool~\cite{liu2020closer} & - & - & 66.7 &94.9 &98.4& 82.5& 0.0 &23.9 &51.8 &70.6& 92.0& 82.3& 76.7& 68.1 &65.0 &61.1  \\ % from ASSA-Net, PosPool original paper, this is on area5, from https://drive.google.com/drive/folders/1MT-262K2m65mkUq077DhrFTMqnM-XdEa

 
% ShellNet~\cite{zhang2019shellnet} &-&-&66.8 & \WM{This is all areas, they don't report area5 !!!}\\ 


% & - & - & - & - & - & - & - & - & - & - & - & - & - 

KPConv~\cite{thomas2019kpconv} & - & 72.8 & 67.1 &92.8 & 97.3 & 82.4 & 0.0 & 23.9 & 58.0 & 69.0 & 81.5 & 91.0 & 75.4 & 75.3 & 66.7 & 58.9 \\ % fro kpconv paper on area5,
ASSANet-L~\cite{qian2021assanet} & - & - & 66.8 & - & - & - & - & - & - & - & - & - & - & - & - & -  \\ % from ASSA-Net verifeid at area5
Point Transformer~\cite{zhao2021pointtransformer} & 90.8 & 76.5 & 70.4 & 94.0 & 98.5 & 86.3 & 0.0 & 38.0 & 63.4 & 74.3 & 89.1 & 82.4 & 74.3 & 80.2 & 76.0 & 59.3\\ % from pointTransofrmer verified at area5 
PatchFormer~\cite{cheng2022patchformer}  & - & - & 68.1 & - & - & - & - & - & - & - & - & - & - & - & - & -  \\ % from pointTransofrmer 
	
RepSurf-U~\cite{ran2022surface} & 90.2& 76.0 & 68.9 & - & - & - & - & - & - & - & - & - & - & - & - & - \\
CBL~\cite{Tang2022ContrastiveBL} & 90.6 & 75.2 & 69.4 & 93.9 & 98.4 & 84.2 & 0.0 & 37.0 & 57.7 & 71.9 & 91.7 & 81.8 & 77.8 & 75.6 & 69.1 & 62.9 \\
Fast PointTransformer~\cite{park2022fpt}  & - & 77.4 & 70.1 & - & - & - & - & - & - & - & - & - & - & - & - & -   \\
StratifiedFormer~\cite{lai2022stratified}  & 91.5 & 78.1 & 72.0 & - & - & - & - & - & - & - & - & - & - & - & - & -  \\ % from StratifiedTransofrmer verified at area5 

\midrule
\gr PointNet++~\cite{qi2017pointnet2} & 83.0 & - & 53.5 & - & - & - & - & - & - & - & - & - & - & - & - & -\\ % from ASSA-Net
\gr \textbf{PointNeXt-S (ours)}					&87.9$\pm$0.3	&70.0$\pm$0.7	&63.4$\pm$0.8	&93.9	&98.3	&80.4	&0.0	&22.7	&49.1	&64.9	&80.4	&88.8	&61.6	&70.2	&59.7	&53.4\\
\gr \textbf{PointNeXt-B (ours)} 		&89.4$\pm$0.1	&73.7$\pm$0.6	&67.3$\pm$0.2	&93.5	&98.4	&82.5	&0.0	&21.7	&57.8	&71.0	&81.2	&90.1	&74.2	&75.0	&72.2	&57.4\\
\gr \textbf{PointNeXt-L (ours)}		&90.0$\pm$0.1	&75.3$\pm$0.8	&69.0$\pm$0.5	&94.0	&98.5	&83.5	&0.0	&30.3	&57.3	&74.2	&82.1	&91.2	&74.5	&75.5	&76.7	&58.9\\
\gr \textbf{PointNeXt-XL (ours)} &90.6$\pm$0.1	&76.8$\pm$0.7	&70.5$\pm$0.3	&94.2	&98.5	&84.4	&0.0	&37.7	&59.3	&74.0	&83.1	&91.6	&77.4	&77.2	&78.8	&60.6\\
\bottomrule[1pt]
\end{tabular}}
\end{table*}

==> tables/s3dis_scannet.tex <==
\begin{wraptable}{b}{0.75\textwidth}
\vspace{-1.3em}
\small
\centering
\caption{\textbf{Semantic segmentation on S3DIS with 6-fold cross-validation.} The improvements of our PointNeXt over PointNet++~\cite{qi2017pointnet2} are highlighted in \hl{green} color. Methods are in chronological order.}
\label{tab:s3dis_6fold}
\vspace{-0.5em}
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{ l | l l l |c c c}
\toprule
\textbf{Method} & mIoU & OA & mAcc  & Params.  & FLOPs  & Throughput\\ 
 & (\%) & (\%) & (\%) & M  & G & (ins./sec.) \\ % & G
\midrule
PointNet~\cite{qi2017pointnet} & 47.6 & 78.5 & 66.2  & 3.6 & 35.5 & 162 \\ % from point cnn on all areas
PointCNN~\cite{li2018pointcnn}& 65.4 & 88.1 & 75.6  & 0.6 & - & -\\ % confirmed on the sup material on PointCNN
DGCNN~\cite{wang2019dgcnn}  & 56.1 & 84.1 & -  & 1.3 & - & 8 \\  % 6 folds on all areas from PCT
% RSNet~\cite{huang2018rsnet} & -- & 66.5 & 56.5 & - & - & - \\ % 6 folds from RS-Net sup material, oa-macc-miou
DeepGCN~\cite{li2019deepgcns} & 60.0  & 85.9 & -& 3.6 & - & 3 \\ % confirmed on all areas from Deep-GCN main table
% SPGraph~\cite{landrieu2018spg} & 85.5 & 73.0 & 62.1 & - & - & -\\ % confirmed on all areas from SPGraph, oa-macc-miou
% PAT~\cite{yang2019modeling} & -- & 76.5 & 64.3 & - & - & -\\ % confirmed on all areas from PAT, oa-macc-miou
% PointWeb~\cite{zhao2019pointweb} & 87.3 & 76.2 & 66.7& - & - & - \\ % confirmed on PointWeb all areas, oa-macc-miou
% ShellNet~\cite{zhang2019shellnet} & 66.8 & 87.1 & - & - & - & - \\ % confirmed on all areas
KPConv~\cite{thomas2019kpconv} & 70.6 & - & 79.1  & 15.0 & - & 30  \\ % confirmed on all throughput 1 areas from KPconv and randlenet In open3dml paras =18.3
RandLA-Net~\cite{hu2020randla} & 70.0 & 88.0 & 82.0  & 1.3  & 5.8 & 159 \\ % confirmed on all areas from randlenet throughput Throughput (ins./s): 14.447360277710908  5.76    2.84    1.300
% SCF-Net~\cite{fan2021scf} & 88.4 & 82.7 & 71.6 \\ %  scf net , corrected from SCF-Net confirmed on all areas, oa-macc-miou
BAAF-Net~\cite{qiu2021baaf} & 72.2 & 88.9 & \textbf{83.1}  & 5.0 & - & 10 \\ % confirmed on all areas from BAAF-Net
Point Transformer~\cite{zhao2021pointtransformer} & 73.5 & 90.2 & 81.9 & 7.8 & 5.6  & 34 \\ % confirmed on all areas from Transformer, flops=& 5.64
CBL~\cite{Tang2022ContrastiveBL} & 73.1 & 89.6 & 79.4 & 18.6  &- & -\\ %18628861
% RepSurf-U~\cite{ran2022surface} & 90.9 & 82.6 & 74.3 & 0.976 & -\\, oa-macc-miou
\midrule
\gr
PointNet++~\cite{qi2017pointnet2}	 &  54.5 & 81.0 & 67.1 & 1.0 & 7.2 & 186 \\ % from point cnn,
\gr
\textbf{PointNeXt-S (ours)} & \reshll{68.0}{+}{13.5} & \reshll{87.4}{+}{6.4} & \reshll{77.3}{+}{10.2} & 0.8  & 3.6 & \textbf{227} \\
\gr
\textbf{PointNeXt-B (ours)} & \reshll{71.5}{+}{17.0} & \reshll{88.8}{+}{7.8} & \reshll{80.2}{+}{13.1} & 3.8 & 8.9  & 158\\
\gr
\textbf{PointNeXt-L (ours)} & \reshll{73.9}{+}{19.4}  & \reshll{89.8}{+}{8.8} &  \reshll{82.2}{+}{15.1}& 7.1 & 15.2  & 115 \\
\gr
\textbf{PointNeXt-XL (ours)} & \reshl{\textbf{74.9}}{+}{20.4}  & \reshl{\textbf{90.3}}{+}{9.3} & \reshll{83.0}{+}{15.9}& 41.6 & 84.8 & 46 \\ % flops=& 89.64
\bottomrule[1pt]
\end{tabular}}
\end{wraptable}

\begin{table}
% \tabcolsep=0.15cm
\small
\centering
\caption{Results on ScanNetv2 for semantic segmentation. More results and analysis}
\label{tab:scannet}
% \begin{footnotesize}
\begin{tabular}{l | c | c c }
\hline
\toprule Method & Input & Val mIoU & Test mIoU \\
\specialrule{0em}{2pt}{0pt}
\hline
\specialrule{0em}{2pt}{0pt}

PointNet++~\cite{qi2017pointnet2} & point & 53.5 & 55.7\\

3DMV~\cite{dai20183dmv} & point & - & 48.4 \\

PanopticFusion~\cite{narita2019panopticfusion} & point & - & 52.9 \\

PointCNN~\cite{li2018pointcnn} & point & - & 45.8 \\

PointConv~\cite{wu2019pointconv} & point & 61.0 & 66.6 \\


PointASNL~\cite{yan2020pointasnl} & point & 63.5 & 66.6 \\

SegGCN~\cite{lei2020SegGCN} & point & - & 58.9 \\ 

RandLA-Net~\cite{hu2020randla} & point & - & 64.5 \\

KPConv~\cite{thomas2019kpconv} & point & 69.2 & 68.6 \\

JSENet~\cite{hu2020jsenet} & point & - & 69.9 \\

FusionNet~\cite{zhang2020deep} & point & - & 68.8 \\

PointTransformer~\cite{zhao2021pointtransformer} & point & 70.6 & - \\

SparseConvNet~\cite{3DSemanticSegmentationWithSubmanifoldSparseConvNet} & voxel & 69.3 & 72.5 \\

MinkowskiNet~\cite{choy20194d} & voxel & 72.2 & 73.6 \\

\specialrule{0em}{2pt}{0pt}
\hline
\specialrule{0em}{2pt}{0pt}

Ours & point & \textbf{72.5} & \textbf{71.2} \\

% Ours (w/ ensemble) & point & \textbf{74.8} & \textbf{74.7} \\

% Ours-S & point & 72.6 & 71.5 \\
% Ours-L & point & 74.2 & 73.4 \\

% %\hline
% \specialrule{0em}{2pt}{0pt} 
% \hline
% \specialrule{0em}{2pt}{0pt}

\bottomrule                         

\end{tabular}
% \end{footnotesize}

\vspace{-0.5cm}
\end{table}





==> tables/scannet.tex <==
\begin{table}
% \tabcolsep=0.15cm
\small
\centering
\caption{Results on ScanNetv2 for semantic segmentation. More results and analysis}
\label{tab:scannet}
% \begin{footnotesize}
\begin{tabular}{l | c | c c }
\hline
\toprule Method & Input & Val mIoU & Test mIoU \\
\specialrule{0em}{2pt}{0pt}
\hline
\specialrule{0em}{2pt}{0pt}

PointNet++~\cite{qi2017pointnet2} & point & 53.5 & 55.7\\

3DMV~\cite{dai20183dmv} & point & - & 48.4 \\

PanopticFusion~\cite{narita2019panopticfusion} & point & - & 52.9 \\

PointCNN~\cite{li2018pointcnn} & point & - & 45.8 \\

PointConv~\cite{wu2019pointconv} & point & 61.0 & 66.6 \\


PointASNL~\cite{yan2020pointasnl} & point & 63.5 & 66.6 \\

SegGCN~\cite{lei2020SegGCN} & point & - & 58.9 \\ 

RandLA-Net~\cite{hu2020randla} & point & - & 64.5 \\

KPConv~\cite{thomas2019kpconv} & point & 69.2 & 68.6 \\

JSENet~\cite{hu2020jsenet} & point & - & 69.9 \\

FusionNet~\cite{zhang2020deep} & point & - & 68.8 \\

PointTransformer~\cite{zhao2021pointtransformer} & point & 70.6 & - \\

SparseConvNet~\cite{3DSemanticSegmentationWithSubmanifoldSparseConvNet} & voxel & 69.3 & 72.5 \\

MinkowskiNet~\cite{choy20194d} & voxel & 72.2 & 73.6 \\

\specialrule{0em}{2pt}{0pt}
\hline
\specialrule{0em}{2pt}{0pt}

Ours & point & \textbf{72.5} & \textbf{71.2} \\

% Ours (w/ ensemble) & point & \textbf{74.8} & \textbf{74.7} \\

% Ours-S & point & 72.6 & 71.5 \\
% Ours-L & point & 74.2 & 73.4 \\

% %\hline
% \specialrule{0em}{2pt}{0pt}
% \hline
% \specialrule{0em}{2pt}{0pt}

\bottomrule                         

\end{tabular}
% \end{footnotesize}

\vspace{-0.5cm}
\end{table}


==> tables/scanobjectnn.tex <==
\begin{wraptable}{r}{0.7\textwidth}
% \begin{table}[tb]
\vspace{-0.5em}
\small
\centering
\caption{\textbf{Object classification on ScanObjectNN.} 
% We report the average$\pm$std in three random runs.
}
\label{tab:cls_scanobjectNN}
\vspace{-0.7em}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|ll|ccc}
\toprule
\textbf{Method}&OA & mAcc & Params. & FLOPs & Throughput\\ % 
% \textbf{Method} & (\%) & (\%) & (M)  & (ins./sec.)\\ % & G
\midrule
PointNet~\cite{qi2017pointnet}&68.2  &63.4 & 3.5  & 0.9 & \textbf{4212}  \\ % flops=& 
% SpiderCNN~\cite{xu2018spidercnn} &69.8 &73.7 \\
PointCNN~\cite{li2018pointcnn}&78.5  &75.1 & 0.6  & - & 44 \\
DGCNN~\cite{wang2019dgcnn} &78.1 &73.6 & 1.8   & 4.8 & 402  \\  % flops=& 
% BGA-DGCNN~\cite{uy2019revisiting} &75.7 &79.7 \\
% BGA-PN++~\cite{uy2019revisiting} &77.5 &80.2 \\
% DRNet~\cite{qiu2021dense}  &80.3  &78.0 & - & - & -\\
SimpleView~\cite{goyal2021simpleview} & 80.5 & - &0.8 & - & -\\
PRANet~\cite{cheng2021net}&82.1  & 79.1&  2.3 & - & 493 \\
MVTN~\cite{hamdi2021mvtn} & 82.8 & - & - & - & -\\
% GBNet~\cite{qiu2022gbnet} & 80.5 & 77.8 & 8.8 & - &  194\\
PointMLP~\cite{ma2022pointmlp}  & $85.4\pm1.3$ & $83.9\pm1.5$ & 13.2 & 31.4 & 191\\
% DeltaNet~\cite{Wiersma2022DeltaConv} & 84.7 &  \\
% RepSurf-U~\cite{ran2022surface} & \textbf{86.0} & 83.1 & 6.8 & - \\  
\midrule
\gr PointNet++~\cite{qi2017pointnet2} & 77.9 &75.4 & 1.5  & 1.7 & 1872 \\
\gr \textbf{PointNeXt-S (ours)} & \reshll{$\textbf{87.7}\pm0.4$}{+}{9.8}  &  
\reshll{$\textbf{85.8}\pm0.6$}{+}{10.4} & 1.4  & 1.6 & 2040 \\
\bottomrule
\end{tabular}
}
% \end{table}
\vspace{-2em}
\end{wraptable}

==> tables/semantickitti.tex <==
SemanticKITTI Segmentation 

###############################################3
\begin{table}[ht]
{\Huge
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l|c |c| c| c| c| c| c |c |c| c| c| c| c| c| c| c| c| c| c| c}
% \begin{tabular}{l|c c c c c c c c c c c c c c c c c c c c}

\hline 
Method & \begin{sideways} Mean IoU \end{sideways} 
& \begin{sideways} Car \end{sideways} 
& \begin{sideways} Bicycle \end{sideways} 
& \begin{sideways} Motorcycle \end{sideways} 
& \begin{sideways} Truck \end{sideways} 
& \begin{sideways} Other-vehicle \end{sideways} 
& \begin{sideways} Person \end{sideways} 
& \begin{sideways} Bicyclist \end{sideways} 
& \begin{sideways} Motorcyclist \end{sideways} 
& \begin{sideways} Road \end{sideways} 
& \begin{sideways} Parking \end{sideways} 
& \begin{sideways} Sidewalk \end{sideways} 
& \begin{sideways} Other-ground \end{sideways} 
& \begin{sideways} Building \end{sideways} 
& \begin{sideways} Fence \end{sideways} 
& \begin{sideways} Vegetation \end{sideways} 
& \begin{sideways} Trunk \end{sideways} 
& \begin{sideways} Terrain \end{sideways} 
& \begin{sideways} Pole \end{sideways} 
& \begin{sideways} Traffic-sign \end{sideways}\\ 
% & \begin{sideways} FPS (Hz) \end{sideways}  \\
% \hline

% \textbf{ClassRatio} &-&3.82 &0.02 &0.04 &0.18 &0.23 &0.04 &0.01 &0.01 &16.60 &1.19 &11.75 &0.44 &15.88 &6.97 &32.83 &0.68 &8.93 &0.31 &0.08 \\
\hline
PointNet \cite{qi2017pointnet}
& 14.6 & 61.6 & 35.7 & 15.8 & 1.4 & 41.4 & 46.3 & 0.1 & 1.3 & 0.3 & 0.8 & 31.0 & 4.6 & 17.6 & 0.2 & 0.2 & 0.0 & 12.9 & 2.4  & 3.7 \\


S-BKI \cite{gan2020bayesian} %correct
& $51.3$ & $83.8$ & $30.6$ & $43.0$ & $26.0$ & $19.6$ & $8.5$ & $3.4$ & $0.0$ & $92.6$ & $65.3$ & $77.4$ & $30.1$ & $89.7$ & $63.7$ & $83.4$ & $64.3$ & $67.4$ & $58.6$ & $67.1$  \\
RangeNet++ \cite{milioto2019rangenet++} %correct
& $52.2$ & $91.4$ & $25.7$ & $34.4$ & $25.7$ & $23.0$ & $38.3$ & $38.8$ & $4.8$ & $91.8$ & $65.0$ & $75.2$ & $27.8$ & $87.4$ & $58.6$ & $80.5$ & $55.1$ & $64.6$ & $47.9$ & $55.9$  \\
LatticeNet  \cite{rosu2019latticenet} %correct
& $52.9$ & $92.9$ & $16.6$ & $22.2$ & $26.6$ & $21.4$ & $35.6$ & $43.0$ & $46.0$ & $90.0$ & $59.4$ & $74.1$ & $22.0$ & $88.2$ & $58.8$ & $81.7$ & $63.6$ & $63.1$ & $51.9$ & $48.4$ \\
RandLA-Net \cite{hu2020randla} %correct
& $53.9$ & $94.2$ & $26.0$ & $25.8$ & $40.1$ & $38.9$ & $49.2$ & $48.2$ & $7.2$ & $90.7$ & $60.3$ & $73.7$ & $20.4$ & $86.9$ & $56.3$ & $81.4$ & $61.3$ & $66.8$ & $49.2$ & $47.7$  \\
PolarNet \cite{zhang2020polarnet} %correct
& $54.3$ & $93.8$ & $40.3$ & $30.1$ & $22.9$ & $28.5$ & $43.2$ & $40.2$ & $5.6$ & $90.8$ & $61.7$ & $74.4$ & $21.7$ & $90.0$ & $61.3$ & $84.0$ & $65.5$ & $67.8$ & $51.8$ & $57.5$  \\
MinkNet42 \cite{choy20194d} %correct
& $54.3$ &  $94.3$ & $23.1$ & $26.2$ & $26.1$ & $36.7$ & $43.1$ & $36.4$ & $7.9$ & $91.1$ & $63.8$ & $69.7$ & $29.3$ & $92.7$ & $57.1$ & $83.7$ & $68.4$ & $64.7$ & $57.3$ & $60.1$ \\ %$3.4 HZ$
3D-MiniNet \cite{alonso2020MiniNet3D} %correct
& $55.8$ & $90.5$ & $42.3$ & $42.1$ & $28.5$ & $29.4$ & $47.8$ & $44.1$ & $14.5$ & $91.6$ & $64.2$ & $74.5$ & $25.4$ & $89.4$ & $60.8$ & $82.8$ & $60.8$ & $66.7$ & $48.0$ & $56.6$ \\
% SqueezeSegV3 \cite{xu2020squeezesegv3} %correct 
% & $55.9$ & $92.5$ & $38.7$ & $36.5$ & $29.6$ & $33.0$ & $45.6$ & $46.2$ & $20.1$ & $91.7$ & $63.4$ & $74.8$ & $26.4$ & $89.0$ & $59.4$ & $82.0$ & $58.7$ & $65.4$ & $49.6$ & $58.9$ \\
Kpconv \cite{thomas2019kpconv} %correct
& $58.8$ & $96.0$ & $30.2$ & $42.5$ & $33.4$ & $44.3$ & $61.5$ & $61.6$ & $11.8$ & $88.8$ & $61.3$ & $72.7$ & $31.6$ & $90.5$ & $64.2$ & $84.8$ & $69.2$ & $69.1$ & $56.4$ & $47.4$ \\ 
SalsaNext \cite{cortinhal2020salsanext}
& $59.5$ & $91.9$ & $48.3$ & $38.6$ & $38.9$ & $31.9$ & $60.2$ & $59.0$ & $19.4$ & $91.7$ & $63.7$ & $75.8$ & $29.1$ & $90.2$ & $64.2$ & $81.8$ & $63.6$ & $66.5$ & $54.3$ & $62.1$    \\
BAAF-Net~\cite{qiu2021semantic}
& $59.9$ & $90.9$ & $74.4$ & $62.2$ & $23.6$ & $89.$ & $95.4$ & $48.7$ & $31.8$ & $35.5$ & $46.7$ & $82.7$ & $63.4$ & $67.9$ & $49.5$ & $55.7$ & $53.0$ & $60.8$ & $53.7$ & $52.0$ \\
FusionNet   \cite{zhang2020deep}
& $61.3$  & $95.3$ & $47.5$ & $37.7$ & $41.8$ & $34.5$ & $59.5$ & $56.8$ & $11.9$ & $91.8$ & $68.8$ & $77.1$ & $30.8$ & $92.5$ & $69.4$ & $84.5$ & $69.8$ & $68.5$ & $60.4$ & $66.5$\\
% Cylinder3D  \cite{zhou2020cylinder3d}
% & $61.8$ & $\textbf{96.1}$ & $54.2$ & $47.6$ & $38.6$ & $\textbf{45.0}$ & $65.1$ & $63.5$ & $13.6$ & $91.2$ & $62.2$ & $75.2$ & $18.7$ & $89.6$ & $61.6$ & $85.4$ & $69.7$ & $69.3$ & $\textbf{62.6}$ & $64.7$\\
KPRNet    \cite{kochanov2020kprnet}
& $63.1$ & $95.5$ & $54.1$ & $47.9$ & $23.6$ & $42.6$ & $65.9$ & $65.0$ & $16.5$ & $93.2$ & $73.9$ & $80.6$ & $30.2$ & $91.7$ & $68.4$ & $85.7$ & $69.8$ & $71.2$ & $58.7$ & $64.1$\\
SPVNAS    \cite{tang2020searching}
& $67.0$ & $97.2$ & $50.6$ & $50.4$ & $56.6$ & $58.0$ & $67.4$ & $67.1$ & $50.3$ & $90.2$ & $67.6$ & $75.4$ & $21.8$ & $91.6$ & $66.9$ & $86.1$ & $73.4$ & $71.0$ & $64.3$ & $67.3$\\
% \cline{2-23} 
 AF$^2$-S3Net \cite{cheng20212} 
& $69.7$ & $94.5$ & $65.4$ & $86.8$ & $39.2$ & $41.1$ & $80.7$ & $80.4$ & $74.3$ & $91.3$ & $68.8$ & $72.5$ & $53.5$ & $87.9$ & $63.2$ & $70.2$ & $68.5$ & $53.7$ & $61.5$ & $71.0$ \\
\hline
PointNet++ & $47.16$ & $73.9$ & $28.6$ & $23.7$ & $34.0$ & $23.6$ & $5.8$ & $6.4$ & $3.6$ & $88.1$ & $56.3$ & $72.3$ & $24.2$ & $88.4$ & $60.7$ & $80.8$ & $62.8$ & $67.0$ & $50.3$ & $45.5$ \\

\hline
PointNet++~\cite{qi2017pointnet2} %correct
& 20.1 & 72.0 & 41.8 & 18.7 & 5.6 & 62.3 & 53.7 & 0.9 & 1.9 & 0.2 & 0.2 & 46.5 & 13.8 & 30.0 & 0.9 & 1.0 & 0.0 &16.9 & 6.0 & 8.9 \\
\gr \textbf{PointNeXt (ours)} & TBD \\

\hline
\end{tabular}}
\caption{Segmentation IoU (\%) results on the SemanticKITTI test dataset.}
\label{bigtable}}
\end{table} 

